General Debiasing for Graph-based Collaborative Filtering via Adversarial Graph Dropout

Graph neural networks (GNNs) have shown impressive performance in recommender systems, particularly in collaborative filtering (CF). The key lies in aggregating neighborhood information on a user-item interaction graph to enhance user/item representations. However, we have discovered that this aggregation mechanism comes with a drawback, which amplifies biases present in the interaction graph. For instance, a user's interactions with items can be driven by both unbiased true interest and various biased factors like item popularity or exposure. However, the current aggregation approach combines all information, both biased and unbiased, leading to biased representation learning. Consequently, graph-based recommenders can learn distorted views of users/items, hindering the modeling of their true preferences and generalizations. To address this issue, we introduce a novel framework called Adversarial Graph Dropout (AdvDrop). It differentiates between unbiased and biased interactions, enabling unbiased representation learning. For each user/item, AdvDrop employs adversarial learning to split the neighborhood into two views: one with bias-mitigated interactions and the other with bias-aware interactions. After view-specific aggregation, AdvDrop ensures that the bias-mitigated and bias-aware representations remain invariant, shielding them from the influence of bias. We validate AdvDrop's effectiveness on five public datasets that cover both general and specific biases, demonstrating significant improvements. Furthermore, our method exhibits meaningful separation of subgraphs and achieves unbiased representations for graph-based CF models, as revealed by in-depth analysis. Our code is publicly available at https://github.com/Arthurma71/AdvDrop.

==> backup/1_introduction.tex <==
\section{Introduction}
Personalized recommender systems play a vital role in the information explosion era of the web \cite{youtuberec, seqrec}. 
Collaborative filtering (CF), which primarily focuses on learning high-quality user/item representations from historical interactions, is the most widely used among various recommendation techniques due to the ease of data collection \cite{NCL, AutoCF}.
Recently, by naturally modeling the user-item interactions as a bipartite graph structure and incorporating the idea of graph neural networks (GNNs) in CF, numerous graph-based CF models have been developed, such as NGCF \cite{NGCF}, PinSage \cite{PinSage}, LightGCN \cite{LightGCN}, and UltraGCN \cite{UltraGCN}. 
By iteratively aggregating high-order collaborative signals, these state-of-the-art graph-based CF models incorporate information from multi-hop neighbors into representation learning \cite{GraphSage, MCCF, LR-GCCF, SGL}, thereby significantly enhancing their recommendation performance.

Despite their impressive performance of graph-based CF models, observed user-item bipartite graphs adopted by recommenders ubiquitously contain biased interactions, including noise-injected observations \cite{Survey_bias} and the well-known missing-not-at-random issue \cite{Missing-Not-At-Random}. 
Worse still, the multiple-layer structure of graph-based recommenders can even exacerbate these biases through neighborhood aggregation \cite{FPC, unfairness}.
Specifically, popular users/items, as highly centralized nodes in the user-item graph, dominate message passing and unintentionally exert a larger impact on representation learning \cite{APDA};
User conformity and sensitive attributes can also over-aggregate via the multi-hop graph structure, leading to undesirable clusters of representations - a manifestation of conformity bias \cite{DICE} and fairness issues \cite{CFC,survey_fair}.
These model biases, inherited from various data biases, are inevitably amplified during the graph-based CF optimization process \cite{r-adjNorm}, thereby limiting the out-of-distribution generalization ability of learned representations and making recommender learning more vulnerable to data bias \cite{DecRS}.
Moreover, biases—either predefined or latent confounders—found in real-world scenarios, which are typically studied independently \cite{InvPref, CausPref}, present additional challenges. 
Even though specific bias-mitigating research in CF has proliferated, the exploration of general debiasing, a more practical and important setting, is far from being well-explored in literature \cite{COR}.

\begin{figure*}[t]
	\centering
	\subcaptionbox{User Gender (MF)\label{fig:gender_mf}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/0_epoch_499_adv_0_user_attribute_0_gamma_0.21960332989692688.png}}
	\subcaptionbox{User Gender (LightGCN-2L)\label{fig:gender_LightGCN2}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/2_epoch_499_adv_0_user_attribute_0_gamma_0.4465178847312927.png}}
    \subcaptionbox{User Gender (LightGCN-4L) \label{fig:gender_LightGCN4}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/4_epoch_319_adv_0_user_attribute_0_gamma_0.45302748680114746.png}}
	\subcaptionbox{User Gender (AdvDrop)\label{fig:gender_AdvDrop}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/advdrop_epoch_499_adv_0_user_attribute_0_gamma_0.004467576742172241.png}}

	\subcaptionbox{Item Popularity (MF)\label{fig:pop_mf}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/0_epoch_499_adv_0_item_attribute_4_gamma_0.18391433358192444.png}}
	\subcaptionbox{Item Popularity (LightGCN-2L)\label{fig:pop_LightGCN2}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/2_epoch_499_adv_0_item_attribute_4_gamma_0.10660887509584427.png}}
    \subcaptionbox{Item Popularity  (LightGCN-4L)\label{fig:pop_LightGCN4}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/4_epoch_319_adv_0_item_attribute_4_gamma_0.11752838641405106.png}}
	\subcaptionbox{Item Popularity (AdvDrop)\label{fig:pop_AdvDrop}}{
	    % \vspace{-6pt}
		\includegraphics[width=0.23\linewidth]{figures/fig1/advdrop_epoch_499_adv_0_item_attribute_4_gamma_0.011166826821863651.png}}
	%\vspace{-10pt}
	\caption{T-SNE \cite{t-sne} visualizations of user/item representations learned by MF \cite{BPR}, LightGCN \cite{LightGCN}, and our proposed model, AdvDrop. The subfigures (\ref{fig:gender_mf}-\ref{fig:gender_AdvDrop}) and (\ref{fig:pop_mf}-\ref{fig:pop_AdvDrop}) illustrate the representation spaces corresponding to different user genders and varying item popularity levels, respectively, under the head, mid, and tail group categorizations.}
	\label{fig:toy-example}
	\vspace{-10pt}
\end{figure*}

\begin{figure}
      \centering
      \includegraphics[width=0.85\linewidth]{figures/intro/rec_perf.png}
      \caption{Recommendation Performance}
      \label{fig:rec_perf}
\end{figure}

We further illustrate the bias amplification issue of graph-based CF models in CF with a concrete example, as shown in Fig. \ref{fig:toy-example} and Fig. \ref{fig:rec_perf}. 
Here we show the comparison of a well-known graph-based CF method, LightGCN \cite{LightGCN} with two and four propagation layers (\ie LightGCN-2L, LightGCN-4L), and traditional matrix factorization (MF) regarding model performance, learned representations, and measurement of fairness bias - prediction bias $\gamma_{bias}$ \cite{CFC} on a public dataset Coat. 
As depicted in Fig. \ref{fig:toy-example}, the points represent T-SNE visualization \cite{t-sne} of user or item representations are colored according to user gender, which represents a sensitive attribute of the user. 
Item embeddings are colored according to popularity, a common bias factor. 
Prediction bias measures the average prediction disparity w.r.t different user/item attributes, which can be depicted as a quantifier for recommendation bias (see definition in Section \ref{sec:exp}).
It is observed that although GNN outperforms MF on recommendation metrics as shown in figure \ref{fig:a}, the resulting representations and prediction suffer more severely from model inherent bias. User embeddings are more compactly clustered comparing figure \ref{fig:c} to figure \ref{fig:b}, which is at higher risk of leaking sensitive information. Tail items cluster at the origin while head items spread outwardly in figure \ref{fig:e}, which illustrates the undesired domination of popular items in GNN compared to figure \ref{fig:d}. Quantitatively, the prediction bias of LightGCN for user gender and item popularity are both significantly higher. 
This example clearly shows CF methods with GNN as a backbone are more heavily biased than their MF counterparts. 
Past research \cite{bc_loss} indicates GNN-based CF methods may directly suffer in out-of-distribution performance when facing heavily sparse and biased graphs, and our experiments show that some debiasing methods designed for traditional CF suffer in performance when adapted to graph-based scenarios.
This example clearly proves that the graph-based CF model will aggravate the issues of popularity bias and unfairness with the stacking of layers.

Motivated by the aforementioned challenge, we argue that an ideal debiasing strategy should be capable of alleviating both general bias and bias amplification that are intrinsic in the model itself, rather than concentrating only on a specific data bias. 
With the goal of general debiasing for graph-based CF models, model debiasing strategies should shield the representation learning from the influence of biased neighborhood propagation.
In the case of popularity debiasing, for instance, unbiased user representation is expected to be invariant when randomly removing graph edges with popular or unpopular neighbors.
This forces the debiasing model to learn bias-agnostic features regardless of biased graph structures. 
However, existing literature on model debiasing has been conducted to randomly sample interaction subgraphs \cite{SGL} or alter the message passing scheme \cite{APDA} in accordance with a specific predefined bias, leaving the unknown general bias untouched.
This inspires us to develop a model debiasing strategy for automatically identifying and eliminating general bias during neighborhood aggregation.

Toward this end, we incorporate Adversarial Graph Dropout into graph-based CF models and propose a novel \textbf{AdvDrop} framework for general debias in recommender systems. 
Specifically, for each user/item, AdvDrop generates bias-mitigated and bias-augmented subgraphs as graph structure input and enforces that its representations derived from different subgraphs be invariant to one another.
By framing the bias-aware subgraph generation as the bias identification stage and invariant representation learning as the debiasing stage, our AdvDrop is distilled into an iterative optimization process under a min-max framework:
\begin{itemize}
    \item In the debiased representation learning stage, AdvDrop updates user/item representations by jointly optimizing the recommendation objective and \textbf{minimizing} the discrepancy between the representations learned from sampled bias-augmented and bias-mitigated subgraphs.
    \item In the bias identification stage, AdvDrop determines the bias distributions of interaction in an adversarial manner by \textbf{maximizing} discrepancy between user/item representations that come from sampled subgraphs.
\end{itemize}

Benefiting from the above adversarial learning scheme, AdvDrop is able to simultaneously discover various biases during neighborhood aggregation and achieves unbiased representation learning for graph-based CF models. 
AdvDrop, a simple yet effective plugin, can be easily applied to current graph-based CF backbones, and we implement it on the cutting-edge model LightGCN \cite{LightGCN}.
Extensive experiments show that our AdvDrop significantly outperforms the state-of-the-art baselines on both general bias and multiple specific biases scenarios, where the bias factors are either unknown or pre-defined. 
These universal improvements in recommendation accuracy and visualizations of bias distributions clearly demonstrate the effectiveness of AdvDrop.

The main contributions of this paper are as follows:
\begin{itemize}
    \item We uncover the problem of model inherent bias for graph-based CF models, 
    which is important and widespread but far from being well-studied.
    \item We propose a novel debiasing framework in an adversarial manner, named as AdvDrop, which forces the representations learned from different subgraphs generated by bias-aware dropout to be consistent with each other.
    \item Through extensive experiments including both general and specific bias scenarios as well as visualization of learned representations and bias distributions, we validate the universal effectiveness of AdvDrop.
\end{itemize}


==> backup/4_experiment.tex <==
\section{Experiments}
\label{sec:exp}

In order to verify the effectiveness of AdvDrop and understand the reason for its superior performance, we conduct extensive experiments to answer the following research questions:
\begin{itemize}[leftmargin=*]
   \item \textbf{RQ1:} How does Advdrop perform compared with other baseline models on General Debiasing datasets?
   \wx{\item \textbf{RQ2:} Can Advdrop successfully address various specific biases?}
   \item \textbf{RQ3:} What is the crucial information that the adversarial learning scheme in Advdrop captures, and how does it affect the learned representations? 
\end{itemize}



\begin{table*}[ht]
\caption{Comparison of general debiasing performance on Coat, Yahoo, and KuaiRec. The improvements over the baselines are statistically significant at 0.05 level ($p$-value $\ll 0.05$).}
\vspace{-10pt}
\label{tab:overall}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc||cc|cc}
\hline
\multicolumn{1}{c|}{Dataset} & \multicolumn{4}{c|}{Coat}       & \multicolumn{4}{c||}{Yahoo}   & \multicolumn{4}{c}{KuaiRec} \\
\hline
\multirow{2}{*}{TopK}&
  \multicolumn{2}{c|}{NDCG} &
  \multicolumn{2}{c|}{Recall} &
  \multicolumn{2}{c|}{NDCG} &
  \multicolumn{2}{c||}{Recall} &
  \multicolumn{2}{c|}{NDCG} &
  \multicolumn{2}{c}{Recall} \\\cline{2-13} & Top3 & Top5   & Top3 & Top5   & Top3 & Top5   & Top3 & Top5   & Top20 & Top30    & Top20 & Top30  \\
\hline
LightGCN              & 0.499 & 0.523 & 0.394 & 0.519 &0.610 & 0.673 & \underline{0.640} & 0.804  & 0.334  & 0.331  & 0.073  & 0.114 \\
IPS-CN             & \underline{0.51}6 & \underline{0.538} & 0.406 & 0.524 & 0.598 & 0.664 & 0.628 & 0.797 & 0.014  & 0.014  & 0.002  & 0.003\\
DR               & 0.506 & 0.524 & \underline{0.416} & 0.534 & \underline{0.611} & \underline{0.677} & 0.637 & \underline{0.805} & 0.037  & 0.035  & 0.010  & 0.013 \\
CVIB & 0.488  & 0.528  & 0.386 & \underline{0.538}  &   0.597 & 0.657  &  0.632  &  0.787  &    \underline{0.342} & \underline{0.336}    & \underline{0.079}  &  \underline{0.118} \\
InvPref                & 0.365 & 0.421 & 0.293 & 0.438 & 0.594 & 0.653 & 0.621 & 0.773 & N/A  & N/A  & N/A  & N/A \\
AutoDebias                & 0.502 & 0.529 & 0.401 & 0.527 & 0.601 & 0.658 & 0.627 & 0.782 & 0.327  & 0.316  & 0.072  & 0.105 \\
AdvDrop            & \textbf{0.532}* & \textbf{0.553}* & \textbf{0.418}* & \textbf{0.540}* & \textbf{0.617}* & \textbf{0.681}* & \textbf{0.643}* & \textbf{0.807}* & \textbf{0.362}*  & \textbf{0.351}*  & \textbf{0.089}*  & \textbf{0.130}* \\\hline
Imp. \%              &   2.04\%     &  1.64\%      &   0.48\%     &    0.18\%    &  0.72\%      &    0.56\%    &   0.41\%     &   0.29\%     &   5.39\%      &   4.35\%      &   12.16\%      &   8.70\%    \\
\hline
\end{tabular}}
\vspace{-10pt}
\end{table*}




\begin{table}[ht]
\caption{Performance of dealing with Popularity Bias on Yelp2018.}
\vspace{-10pt}
\label{tab:popularity}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
\multicolumn{1}{c|}{Test Split} & \multicolumn{2}{c|}{Test ID}       & \multicolumn{2}{c}{Test OOD}  \\
\hline
Metrics & NDCG@20 & Recall@20 & NDCG@20 & Recall@20 \\
\hline
LightGCN             & 0.0371 & 0.0527 & 0.0028 & 0.0026 \\
IPS-CN            & 0.0337 & 0.0470 & 0.0033 & 0.0030 \\
CDAN             & \underline{0.0496} & \underline{0.0703} & \underline{0.0037} & \underline{0.0037}\\
sDRO              & 0.0492 &  0.0702 & 0.0035 & 0.0034\\
AdvDrop            & \textbf{0.0608} & \textbf{0.0817} & \textbf{0.0066} & \textbf{0.0073} \\
\hline
\end{tabular}}
\vspace{-10pt}
\end{table}

\begin{table*}[ht]
\caption{Performance of dealing with Fairness Issue on Coat.}
\vspace{-10pt}
\label{tab:fairness}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c}
\hline
% \multicolumn{1}{c|}{Dataset} & \multicolumn{2}{c|}{Test IID}       & \multicolumn{2}{c}{Test OOD}  \\
% \hline
\multirow{2}{*}{Evaluation Metrics}&
  \multicolumn{4}{c|}{Performance Metrics} &
  \multicolumn{3}{c}{Fairness Metric (Prediction Bias)}  \\\cline{2-8} & NDCG@3 & NDCG@5   & Recall@3 & Recall@5   & user gender & item colour &  item gender \\
\hline
MF       & 0.473 & 0.508 & 0.349 & 0.501 & 0.102 & 0.175 & 0.091 \\
LGN       & 0.499 & 0.523 & 0.394 & 0.519 & 0.420 & 0.589  & 0.468 \\
\hline
AdvDrop             & \textbf{0.532} & 0.553 & 0.418 & 0.540 & 0.142 & 0.053 & 0.062 \\
+Embed info             & \underline{0.518} & \textbf{0.560} & \underline{0.418} & \underline{0.578}& 0.052 & 0.032 & 0.046 \\
+Mask info              & 0.512 & \underline{0.554} & \textbf{0.425} & \textbf{0.581} & \underline{0.045} & \underline{0.024} & \underline{0.039}\\
\hline
CFC            & 0.485 & 0.513 & 0.395 & 0.517 & \textbf{0.012} & \textbf{0.011} & \textbf{0.012} \\ 
\hline
\end{tabular}}
\vspace{-10pt}
\end{table*}




\subsection{Experimental Settings}
\textbf{Datasets.} 
We conduct experiments on four real-world benchmark datasets that involves recommendation debias under both general bias and specific bias settings as listed below:
\begin{itemize} [leftmargin = *]
    \item \textbf{Yahoo\cite{Yahoo} \& Coat\cite{schnabel2016recommendations}.} Both datasets are commonly used as benchmark dataset for general debias in recommendation. They both consist of a biased training set of normal user interactions and an unbiased uniform test set collected by a random logging policy. During data collection, users interacts with items by giving ratings (1-5). In our experiments, interactions with scores $\geq$ 4 are considered as positive samples, and negative samples are collected from all possible user-item pairs. 

    \item \textbf{Douban-Movie\cite{Douban}.} This dataset contains user interactions with movies (writing reviews) on a popular site Douban. The interactions are provided along with associated timestamps. We constructed our data following temporal splitting strategy\cite{MengMMO20}. Specifically, we split the time range for data collection into 10 folds, then assign interactions within each fold into training, validation and test sets with a 6:1:3 ratio. 

    \item \textbf{Yelp2018\cite{LightGCN}.} This dataset is adopted from the 2018 edition of the Yelp challenge. Users visiting to local businesses are recorded as interactions. Following previous work\cite{bcloss}, we split the dataset into in-distribution (ID) and out-of-distribtion (OOD) test splits with respect to popularity. 
    
\end{itemize}

Table \ref{tab:dataset-statistics} summarizes the detailed statistics of each dataset.






\vspace{5pt}
\noindent\textbf{Evaluation Metrics.}
To evaluate the performance of the model, we use the following metrics:
\begin{itemize} [leftmargin = *]
    \item \textbf{NDCG@K} measures the ranking quality by discounting importance based on position and is defined as below: 
    \begin{equation*}
    \begin{split}
        DCG_{u}@K &= \sum_{(u,v)\in D_{test}} \frac{I(\hat{r}_{u,i}\leq K)}{\log( \hat{r}_{u,v} + 1)} \\
        NDCG_{u}@K &= \frac{1}{|\Set{U}|}\sum_{ u\in \Set{U} } \frac{DCG_{u}@K}{IDCG_{u}@K},
    \end{split}
    \end{equation*}
    where $D_{test}$ is the test dataset, $\hat{r}_{u,i}$ is the rank of item i in the list of relevant items of u, $\Set{U}$ is the set of all users, and $IDCG_{u}@K$ is the ideal $DCG_{u}@K$.

    \item \textbf{Recall@K} measures the percentage of the recommended items in the user interacted items. The formula is as below:
    \begin{equation*}
    \begin{split}
        Recall_{u}@K &=  \frac{\sum_{(u,i)\in D_{test}} I(\hat{r}_{u,i} \leq K)}{|D^{u}_{test}|} \\
        Recall@K &= \frac{1}{|\Set{U}|}\sum_{ u\in \Set{U} } Recall_{u}@K,
    \end{split}
    \end{equation*}
    where $D^{u}_{test}$ is the set of all interactions of user u in the test dataset $D_{test}$.

    \item \textbf{Prediction bias} measure the level of parity regarding predicted recommendation ratings w.r.t. a given attribute. Prediction bias of a certain user attribution is given by:
    \begin{equation*}
    \begin{split}
        \gamma_{bias} &=  \frac{1}{|\Set{I}|} \sum_{i\in \Set{I}}\max_{\substack{a_1,a_2\in A \\ a_1\neq a_2}}\Big|{\mathrm{Avg}}_{\{u|a_u = a_1\}}(\hat{y}_{ui}) - {\mathrm{Avg}}_{\{v|a_v = a_2\}}(\hat{y}_{vi})\Big|,
    \end{split}
    \end{equation*}
    where $a_1$,$a_2$ are two user attribute labels, $A$ is the set of user attribute labels, and $\Set{I}$ is the set of items. Item attribute's prediction bias can be obtained likewise.
\end{itemize}






\vspace{5pt}
\noindent\textbf{Baselines.}

We adopt various baselines for general debias and representative baselines for specific bias in recommendation. Detail for baselines can be found in appendix \ref{app:baseline}.
\begin{itemize} [leftmargin = *]
\item \textbf{Methods for General Debias }: IPS-CN \cite{gruson2019offline}, DR \cite{wang2019doubly}, CVIB \cite{wang2020information}, and InvPref \cite{wang2022invariant}.


\item \textbf{Methods for Special Bias }: IPS-CN \cite{gruson2019offline} (popularity), CDAN \cite{chen2022co} (popularity), sDRO \cite{wen2022distributionally} (popularity), and CFC \cite{bose2019compositional} (Unfairness).

\end{itemize}


\subsection{General Debiasing Performance (RQ1)}
\noindent \textbf{Motivation.} Existing recommendation debiasing techniques that addresses general bias usually concentrate on unbiased test set constructed from completely missing-at-random (MAR) user feedback. However, real-world scenarios require general debiasing algorithm to yield satisfactory performance when dealing with unidentified shift in distribution of user-item interaction (e.g. temporal shift \& demographic shift). In our settings, we experiment on both traditional MAR setting (Yahoo \& Coat) and temporal shift setting (Douban), whereas no prior information on test distribution is given.

\noindent \textbf{Results.}
Table \ref{tab:overall} reports the general debias performance of AdvDrop compared with various baselines. The best-performing method for each metric are in bold, while the second-best are underlined. From the experiment results, we can make the following observations:
\begin{itemize} [leftmargin = *]
    \item \textbf{AdvDrop consistently outperforms various baselines for general debias across all benchmark datasets.} Specifically, AdvDrop achieves 0.18\% $\sim$ 3.23\% improvements w.r.t NDCG and Recall metrics compared to the baselines on Coat and Yahoo, and a more prominent improvement of 2.62\% $\sim$ 5.65\% on Douban temporal split. We attribute the robustness of AdvDrop regarding different general debias settings to iteratively identifying interaction bias directly from the interaction graph and performing bias removal adversarially, without making prior assumptions of test distribution.
    \item \textbf{General debiasing baselines performs inconsistently regarding MAR settings and temporal-split settings, and some suffer drastically from mode inherent bias.} Compared to AdvDrop that is designed to alleviate both general bias and bias amplification that are intrinsic in the graph-based CF models, baseline models shows limited and inconsistent performance gain in recommendation when applied to GNN backbone. Among the compared baselines, IPS-CN out-performs backbone on small-scale MAR setting of Coat but performs unsatisfactorily on others; DR performs well on MAR settings but fails when applied to temporal distribution shift due to incorrect estimation of observation probability on unknown distribution; CVIB underperforms GNN backbone on Yahoo. These results corroborate the necessity of directly learning interaction bias without making prior assumption on test distribution or factor of bias. Surprisingly, we also found that InvPref with LightGCN as backbone fails to capture the general bias across all dataset, while MF+InvPref could successfully mitigate the bias \cite{wang2022invariant}. We attribute such failure to model inherent bias of GNN backbone, which further highlight the importance of designing general debias models that address both data and model intrinsic bias.
\end{itemize}


\subsection{Performance on Specific Bias (RQ2)}

\noindent \textbf{Motivation.}
Intuitively, general debiasing techniques should be able to address various specific biases that exist in recommendation, performing at par with models designed for specific bias. In order to further validate the ability of AdvDrop, we conduct experiments regrading two common bias-related issues, namely popularity bias and fairness issue. Resolving popularity bias requires model to perform well when facing popularity-related distribution shift, while fairness emphasize both representation-level and prediction-level parity for sensitive user/item attributes. The two scenerios together demands models to achieve OOD generalization while maintaining unbiasedness in prediction and representation.

\subsubsection{AdvDrop for Popularity Bias}
The results for dealing with popularity bias is shown in Table \ref{tab:popularity}. We can observe that AdvDrop achieves significant improvements over original LightGCN backbone on both ID and OOD test sets, outperforming all compared baselines. With further analysis of AdvDrop in section \ref{sec:ablation}, we attributes the ID performance gain mainly to the contrastive objective in Debias Representaion Learning stage, and OOD performance gain to both Debias Representation Learning and Bias Identification. 

\subsubsection{AdvDrop for Fairness} 
\begin{figure}
    \vspace{10pt}
    \subcaptionbox{User Gender (AdvDrop)\label{fig:v_a}}{
    \includegraphics[width=0.45\columnwidth]{figures/AdvDrop_gender.png}}
    \vspace{10pt}
    \subcaptionbox{Item Popularity (AdvDrop)\label{fig:v_b}}{
    \includegraphics[width=0.45\columnwidth]{figures/AdvDrop_pop.png}}
    \vspace{-15pt}
    \caption{Visualization of AdvDrop Embeddings }
    %\vspace{-10pt}
    \label{fig:embed_v}
\end{figure}
The results for dealing with fairness issue is shown in Table \ref{tab:fairness}. We compare both recommendation performance and fairness metric of group-wise prediction bias against backbone models MF \& LightGCN, and a representative baseline for fairness issue, CFC. CFC embody a concentrated reflection of the common techniques applied for recommendation fairness, which strictly impose adversarial constraint on the embedding level that obfuscate sensitive attributes in the sense of fooling a classifer built upon learned representations. In this sense, the prediction bias of CFC can be regarded as a lower bound for fairness metric, regardless of model recommendation performance. We make the following observations:
\begin{itemize} [leftmargin = *]
    \item \textbf{In terms of performance, AdvDrop achieves significant performance gain on top of LightGCN backbone, while maintaining reasonable level of prediction bias level with with MF.} This is in stark contrast with prevalent methods dealing with fairness issue, which suffers model performance in exchange for lowered prediction bias. Moreover, when injecting attribute information at the embedding level (+Embed info) or further imposing constraint on $P_B$ w.r.t. attribute category (+Mask Info), Advdrop can enjoy further improved recommendation performance with lowered prediction bias, which is closer to the lower bound from CFC.

    \item \textbf{In terms of representations, AdvDrop alleviates undesired clustering of user/items with similar sensitive attributes and down-tunes accentuation of popular items during neighbor aggregation.} Specifically, we extend the concept of prediction bias to popularity, treating it as a user/item attribute, and plot T-SNE visualization of learned user/item representions w.r.t each attribute. Such trend is clearly depicted in comparison among \ref{fig:b}, \ref{fig:d} and \ref{fig:v_a} regarding sensitive attribute, and among \ref{fig:c}, \ref{fig:e} and \ref{fig:v_b} regarding popularity. Learned representations from AdvDrop resembles represesntations from MF, which is in accordance with the similar trend of performance in prediction bias.
\end{itemize}

These two above observations together clearly demonstrate that AdvDrop successfully removes harmful intrinsic bias in graph-based CF, which further empowers model generalization performance while promoting fairness of recommendation. 




\subsection{Study of AdvDrop (RQ3)}


\subsubsection{Ablation Study} 
\label{sec:ablation}

To further investigate the effective component of AdvDrop, we conducted ablation study on Yelp2018, shown in table \ref{tab:ablation}. We observe that:
\begin{itemize}  [leftmargin = *]
    \item \textbf{When removing the adversarial learning of $P_B$} (w/o $P_B$), model performance on ID test slightly reduced from 0.817 to 0.781 regarding NDCG@20, while OOD performance reduced more significantly from 0.0073 to 0.0060. Note that such ablated model only utilize the contrastive loss $\Set{L}_{inv}$ from two randomly-dropout views of graph, which resembles recent model designs of RDrop and SGL. The performance gain w.r.t. graph-based backbone can be interpreted as performing data augmentations by constructing random views of original interaction graph.  
    \item \textbf{When further reducing the contrastive learning objective $\Set{L}_{inv}$} 
 (w/o $P_B$ \& $\Set{L}_{inv}$), the model is restricted to perform learning with random graph dropout. This result in model performance to fall below graph-based backbone.
\end{itemize}
These evidences imply that \textbf{superior performance of AdvDrop results from both learning stages}: the Debias Representation Learning stage fundamentally improves representation quality, while the Bias Identification stage actively seeks meaningful bias-related views that further boost model generalization performance. 

\begin{table}[ht]
\caption{Ablation study  AdvDrop on Yelp2018.}
\vspace{-10pt}
\label{tab:ablation}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
\multicolumn{1}{c|}{Test Split} & \multicolumn{2}{c|}{Test ID}       & \multicolumn{2}{c}{Test OOD}  \\
\hline
Metrics & NDCG@20 & Recall@20 & NDCG@20 & Recall@20 \\
\hline
AdvDrop            & \textbf{0.0608}  & \textbf{0.0817}  &\textbf{0.0066} &  \textbf{0.0073}  \\\
w/o $P_B$     & \underline{0.0575} &  \underline{0.0781}& \underline{0.0060} &  \underline{0.0060}\\
w/o $P_B$ \& $\Set{L}_{inv}$      & 0.0371  & 0.0528 & 0.0027  & 0.0024 \\
\hline
\end{tabular}}
\vspace{-10pt}
\end{table}

\subsubsection{Visualization of Bias Measurement Function $P_B$}
To understand the crucial information regarding general bias captured by the Bias Identification stage, we visualize learned bias measurement function $P_B$ with respect to item popularity. Specifically, we sort all items according to item popularity, then split them into four groups from 0 to 3 with ascending popularity. We compute the average $P_B$ of interactions connected to items within each group, shown in figure \ref{fig:mask}. One can observe that only group 3 representing interactions with most popular items has an averaged $P_B$ greater than 0.5, while the average $P_B$ from interactions in other groups falls below 0.5. The average $P_B$ strictly ascends corresponding to group popularity. These observations shows the model learns $P_B$ in a conservative manner around 0.5 while impressively matching the long-tailed nature of user popularity, which indicates the Bias Identification stage can successfully captured information regarding interaction bias.



\begin{figure}
    \vspace{10pt}
    \includegraphics[width=0.8\columnwidth]{figures/mask.png}
    \vspace{-10pt}
    \caption{Visualization of learned bias measurement function $P_B$ w.r.t. item popularity.}
    \vspace{-10pt}
    \label{fig:mask}
\end{figure}



\subsubsection{Interpretation of AdvDrop for Debiased Learning}


\begin{figure}
    \vspace{10pt}
    \includegraphics[width=0.9\columnwidth]{figures/bias_vs_rec.png}
    \vspace{-10pt}
    \caption{Recommendation performance v.s. model bias during training on Coat.}
    \vspace{-15pt}
    \label{fig:bias_rec}
\end{figure}

We finally present a intriguing interpretation of how AdvDrop effectively conduct general debias to achieve superior performance. Figure \ref{fig:bias_rec} shows recommendation performance in terms of NDCG@3 against model bias measured by prediction bias during training on Coat for MF, LightGCN and AdvDrop. One can make the following observations:
\begin{itemize} [leftmargin = *]
    \item For MF and LightGCN, the curve begins from bottom-left and extend monotonically to upper-right, representing MF and LightGCN improve recommendation performance during training while accumulate bias in representation. Curve for LightGCN extends further to upper-left than MF, which corresponds to its superior recommendation performance and more severe model intrinsic bias.
    \item For AdvDrop, the curve does not extend monotonically to upper-right, but instead curves eventually backwards to upper-left. This represents AdvDrop learns to remove harmful prediction bias and improves model performance by iterative optimization. Following the curve, we can depict that recommendation performance first improved at the beginning of bias accumulation, then dropped as bias further accumulated (or at the beginning of bias removal), and finally improves at the end when the bias is removed.
    \item For AdvDrop, the time order between re-improvement of recommendation performances and bias removal differs across different attributes. Specifically, bias removal happened before / at the same time / after performance improvements for item gender, user ages and user/item popularity respectively. This indicates that bias identification and removal in AdvDrop is conducted in an ordered manner, and the superior performance can be attributed to the ensemble of orderly removal for different bias. 
\end{itemize}
Again, these observations clearly depict the bias identification and bias removal process in AdvDrop, accounting for its superiority. The orderly removal of bias in AdvDrop is a interesting phenomena that possibly implies implicit ordering in different recommendation bias, which we'll further explore in future work.



==> backup/5_related_work.tex <==
\section{Related Work}
\textbf{Specific Debiasing in recommender systems}. Recommender systems usually face various bias issues due to the inconsistency between observational behavior data and user's true preferences. The common biases include 1) Popularity Bias 2) Exposure Bias, 3) Conformity Bias, 4) Unfairness.


\noindent \textbf{- Popularity Bias.} Recommender systems unduly favor popular items as popular items are more likely to be exposed and have more chances to be clicked. Traditional popularity debiasing methods include: 1) Regularization-based frameworks \cite{chen2020esam,chen2022co,abdollahpouri2017controlling,wen2022distributionally} balance the trade-off between accuracy and converge by incorporating penalty terms. ESAM \cite{chen2020esam} introduce center-wise clustering, self-training regularization strategies to increase the impact of long-tail items. CDAN \cite{chen2022co} uses Pearson coefficient correlation as regularization to disentangle item property representations from item popularity representation.
2) Sample re-weighting methods \cite{gruson2019offline,bottou2013counterfactual, schnabel2016recommendations, joachims2017unbiased} reweight loss of each instance by reversing the item propensity score in the training set, also knows as IPS. To solving high variance of propensities in IPS methods, many works \cite{gruson2019offline, bottou2013counterfactual} adopt normalization or smoothing penalty to stabilize the model performance. Recent works \cite{wei2021model,wen2022distributionally,xu2021deconfounded,wang2020click} takes inspirations from Stable Learning and Causal Inference: MACR \cite{wei2021model} performs counterfactual inference by formulating a causal graph that assumes popularity bias is caused from the item node to the ranking score. sDRO \cite{wen2022distributionally} adopts Distributionally Robust Optimization (DRO) framework that reduces loss variances for long-tailed data distributions. However, the causal graph and environment information requires heuristic knowledge based on author’s understanding. 

\noindent \textbf{- Exposure Bias.} User behaviours are easily affected by the exposure policy of a recommender system, which deviates user actions from true preference. Two types of methods have been proposed to mitigate exposure bias: 1) Reweighting methods \cite{li2010improving,saito2020unbiased,yu2017selection} treat all the unobserved interactions as negative and reweight them by specifying their confidence score. AMAN \cite{li2010improving} defines the user-item feature similarity as the confidence score. UBPR \cite{saito2020unbiased} proposes a new weighting strategy with propensity score to estimate the confidence. 2) Causal Inference methods \cite{xu2021deconfounded,wang2021clicks,yang2021top} mitigate exposure bias by leveraging counterfactual inference. DCCF \cite{xu2021deconfounded} utilizes one of the causal technique, called forward door criterion, to mitigate the impact of unobserved confounders.


\noindent \textbf{- Conformity Bias.} Conformity bias happens as users in a same group are likely to behave similarly even if the decisions are made against their own preferences. Leading conformity debiasing methods can be roughly categorized into two types: 1) Modeling popularity influence methods \cite{liu2016you, zheng2021disentangling,zhao2022popularity} mitigate conformity bias with the popularity information. CM-C \cite{liu2016you} utilizes previous ratings to estimate and predict unknown ratings, considering group size, cohesion, and unanimity factors. DICE \cite{zheng2021disentangling} disentangle conformity embeddings and interest embeddings in the popularity perspective to enforce the model invariant to conformity bias. 2) Modeling social influence methods \cite{ma2009learning,chaney2015probabilistic,wang2017learning} consider the user’s ratings as user preference and social influence. In particular, PTPMF \cite{wang2017learning} proposes a Probabilistic Matrix Factorization model that considers the distinction of strong and weak social ties to learn personalized preference. 
% SPF \cite{chaney2015probabilistic} introduces a probability model that considers social network information to mitigate the impacts of social influence.



\noindent \textbf{- Unfairness.} Unfairness in recommendation results from the system's tendency to learn biased predictions \& representations w.r.t. user or item groups with certain attributes. The major unfairness mitigating methods can be categorized into three lines. 1) Rebalancing based methods \cite{farnadi2018fairness, rahman2019fairwalk, geyik2019fairness,singh2018fairness}
 are inspired by the success of the rebalancing strategy on the class-imbalance problem. They balance recommendation results w.r.t each sensitive attribute. HyPER \cite{farnadi2018fairness} defines user-user, item-item similarity measurements and considers content, and demographic information to balance the discrepancy among groups. Fairwalk \cite{rahman2019fairwalk} samples random walks on the graph structure to generate debiased embeddings by utilizing sensitive attributes. 2) Regularization-based frameworks \cite{kamishima2017considerations,yao2017beyond,yao2017new} formulate the fairness criteria as a regularizer to reduce discrepancy between groups. IERS \cite{kamishima2017considerations} designs a fairness regularizer that incorporates the expected degree of independence between sensitive attributes and predictions. 3) Adversarial Learning based frameworks\cite{bose2019compositional,zhu2020measuring,beigi2020privacy} alternatively optimize the prediction model and an adversary model for debiasing unfairness. Specifically, CFC \cite{bose2019compositional} train filters for
removing sensitive information against discriminators that
predict sensitive attributes from filtered embeddings.

\noindent \textbf{General Debiasing in recommender systems.} It aims to address multiple underlying data biases in a dataset simutaneously. Without knowing the exact type of bias, general debiasing requires model to yield satisfactory performance on various bias-related distributions. However, general debiasing in recommender systems is still under-explored. In the early stage, DR \cite{wang2019doubly} utilizes a small part of missing-at-random data in the test set to generally debias various biases in the data set. CausE \cite{bonner2018causal} introduces a domain adaption algorithm that learns from a logged data with random exposure. Recent research's interest focus on actively discovering latent bias structure and conducting bias removal \cite{CVIB,InvPref}. Specifically, InvPref \cite{wang2022invariant} propose to learn invariant embeddings and perform environment label assignment alternately. Motivated by recent success of invariant learning in computer vision and natural language processing areas, we believe our work is the first to enforce embedding-level invariance w.r.t. adversarially learned views of interaction graph for general debiasing.
% \subsection{Invariant Learning}
% Invariant learning is of particular interest in machine learning area as data is always collected from different environments. The goal of invariant learning is to enforce invariance across environments and learn robust models that general well under distribution shifts. Existing prevalent methods are achieving invariance through enforcing invariance either (1) in features (2) in predictors or (3) in gradients.  First, invariant class features usually extracting by aligning with adversarial methods. 


% \subsection{Environment Inference}

% Prevalent popularity debiasing strategies in CF roughly fall into four research lines.

% \textbf{Post-processing re-ranking methods} \cite{Calibration,RankALS,rescale,FPC,PC_Reg} are applied to the output of the recommender system without changing the representations of users and items. 
% The purposes of modifying the ranking of models can be various: Calibration \cite{Calibration} ensures that the past interests proportions of users are expected to maintain at the same level; RankALS \cite{RankALS} aims to increase the diversification of recommendation; 
% % Scale \cite{rescale} directly re-scale the predicted scores based on popularity to promote unpopular items; 
% FPC \cite{FPC} investigates the popularity bias in the dynamic recommendation by rescaling the predicted scores.

% \textbf{Regularization-based frameworks} \cite{ESAM,ALS+Reg,Regularized_Optimization,PC_Reg} explore the use of regularization that provides a tunable mechanism for controlling the trade-off between recommendation accuracy and coverage.
% The difference among these methods is the design of penalty terms: 
% ALS+Reg \cite{ALS+Reg} defines intra-list distance as the penalty to achieve the fair recommendation; ESAM \cite{ESAM} introduces the attribute correlation alignment, center-clustering, and self-training regularization to learn good feature representations; sam-reg \cite{Regularized_Optimization} regularizes the biased correlation between user-item relevance and item popularity; Reg \cite{PC_Reg} decouples the item popularity with the model preference predictions.

% \textbf{Sample re-weighting methods} \cite{ips,IPS-C,IPS-CN,Propensity_SVM-Rank,YangCXWBE18,UBPR}, also known as Inverse Propensity Score (IPS) view the item popularity in the training set as the propensity score and exploit its inverse to re-weight loss of each instance.
% To address the high variance of re-weighted loss, many of them \cite{IPS-CN,IPS-C} further employ normalization or smoothing penalty to attain a more stable output.
% However, the unreliability of methods is due to their measurement of the propensity score, leveraging the item frequency but failing to consider interaction-wise popularity bias.

% \textbf{Bias removal by causal inference methods} \cite{CausE,KDCRec, DICE, PDA,DecRS,MACR}, getting inspiration from the recent success of counterfactual inference, specify the role of popularity bias in assumed causal graphs and mitigate the bias effect on the prediction. 
% However, the causal structure is heuristically assumed based on the author's understanding, without any theoretical guarantee.

% BC loss opens up a possibility of conventional debiasing methods in CF that mitigate the popularity bias by enhancing the discriminative power. 
% Recent studies, boosting the discriminative feature spaces by modified softmax loss are mainly discussed in face recognition, where a constant margin is added \cite{ArcFace} to better classify.
% We transfer it in recommendation and compare it with our BC loss in Figure \ref{fig:margin}.

% \begin{figure}[t]
% 	\centering
% 	\subcaptionbox{MF+BC loss\label{fig:tau_mf}}{
% 	    \vspace{-5pt}
% 		\includegraphics[width=0.48\linewidth]{figures/effect_tau_mf.pdf}}
% 	\subcaptionbox{LightGCN+BC loss\label{fig:tau_Lightgcn}}{
% 	    \vspace{-5pt}
% 		\includegraphics[width=0.48\linewidth]{figures/effect_tau_lgn.pdf}}
% 	\vspace{-10pt}
% 	\caption{Temperature $\tau$ sensitivity analysis on Tencent.}
% 	\label{fig:tau}
% 	\vspace{-10pt}
% \end{figure}

